Learning multi-modal generative models with permutation-invariant encoders and tighter variational objectives

Devising deep latent variable models for multi-modal data has been a long-standing theme in machine learning research. Multi-modal Variational Autoencoders (VAEs) have been a popular generative model class that learns latent representations that jointly explain multiple modalities. Various objective functions for such models have been suggested, often motivated as lower bounds on the multi-modal data log-likelihood or from information-theoretic considerations. To encode latent variables from different modality subsets, Product-of-Experts (PoE) or Mixture-of-Experts (MoE) aggregation schemes have been routinely used and shown to yield different trade-offs, for instance, regarding their generative quality or consistency across multiple modalities. In this work, we consider a variational objective that can tightly approximate the data log-likelihood. We develop more flexible aggregation schemes that avoid the inductive biases in PoE or MoE approaches by combining encoded features from different modalities based on permutation-invariant neural networks. Our numerical experiments illustrate trade-offs for multi-modal variational objectives and various aggregation schemes. We show that our variational objective and more flexible aggregation models can become beneficial when one wants to approximate the true joint distribution over observed modalities and latent variables in identifiable models.

==> header_tmlr.tex <==
\RequirePackage{epsfig}
\RequirePackage{amssymb}
\RequirePackage{natbib}
\RequirePackage{graphicx}


\bibliographystyle{abbrvnat}



\usepackage{hyperref}
%\hypersetup{
%  colorlinks = true,
%  citecolor = blue,
 %   linkbordercolor = {white},
%}
%\hypersetup{ hidelinks }

\usepackage{multicol} 
% \setlength{\multicolsep}{6.0pt plus 2.0pt minus 1.5pt}
\setlength{\multicolsep}{0.1pt plus 1pt minus 1.5pt}


%\usepackage{subcaption} 
\usepackage{wrapfig}

\usepackage{booktabs}

\usepackage{graphicx}
\usepackage{subcaption}

\usepackage[page]{appendix}

%usepackage{changes}

\usepackage{mathtools}
\usepackage{algorithm}
\usepackage{algpseudocode}

\usepackage[algo2e,inoutnumbered,algoruled,vlined]{algorithm2e}

\usepackage{enumitem}

\usepackage{accents}
\usepackage{dsfont}
\usepackage{aliascnt}
\usepackage{cleveref}
\makeatletter


%\usepackage{todonotes}

\usepackage{etoc}



\newcommand{\mcn}{\mathcal{N}}%
\newcommand{\mcu}{\mathcal{U}}%
\newcommand{\mcl}{\mathcal{L}}%
\newcommand{\mcz}{\mathcal{Z}}%
\newcommand{\mcs}{\mathcal{S}}%
\newcommand{\mch}{\mathcal{H}}%
\newcommand{\mcp}{\mathcal{P}}%
\newcommand{\mcm}{\mathcal{M}}%
\newcommand{\mca}{\mathcal{A}}%
\newcommand{\mcx}{\mathcal{X}}%
\newcommand{\mcd}{\mathcal{D}}%
\newcommand{\mcc}{\mathcal{C}}%


\newcommand{\rset}{\mathbb{R}}%
\newcommand{\nset}{\mathbb{N}}%

\newcommand{\sm}{\setminus}%

\newcommand{\E}{\mathbb{E}}
\newcommand{\mbm}{\mathbb{M}}%


\newcommand{\msx}{\mathsf{X}}%
\newcommand{\msy}{\mathsf{Y}}%
\newcommand{\msa}{\mathsf{A}}%
\newcommand{\msz}{\mathsf{Z}}%
\newcommand{\msk}{\mathsf{K}}%
\newcommand{\msc}{\mathsf{C}}%
\newcommand{\msp}{\mathsf{P}}%


\newcommand{\KL}{\mathsf{K}\mathsf{L}}%

\newcommand{\B}{\bfseries}

\DeclareMathOperator{\I}{I}%
\DeclareMathOperator{\id}{id}%
\newcommand{\rmd}{\mathrm{d}} % differential
\DeclareMathOperator{\e}{e}%

\DeclareMathOperator{\bz}{\boldsymbol{z}}%
\DeclareMathOperator{\bx}{\boldsymbol{x}}%
\DeclareMathOperator{\bm}{\boldsymbol{m}}%
\DeclareMathOperator{\ba}{\boldsymbol{a}}%

\newcommand{\mfi}{\mathfrak{i}}%


\newcommand{\ind}{\perp\!\!\!\!\perp} 

\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\ifdefined\proof
    \renewenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
\else
    \newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
\fi

\newtheorem{example}{Example} 
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma} 
\newtheorem{proposition}[theorem]{Proposition} 
\newtheorem{remark}[theorem]{Remark}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{axiom}[theorem]{Axiom}
